Discovery and capabilities of guard proxies for CoRE networks

Constrained RESTful Environments tolerate and even benefit from proxy services. We explore the concept of proxies installed at entry points to constrained networks without any unified management. We sketch proxies of different levels of intrusiveness into applications, their announcement and discovery, and compare their theoretical capabilities in mitigating the effects of undesired traffic that can otherwise exhaust the environment's constrained resources.

==> Makefile <==
document.pdf: document.tex body.tex tab-effects.tex bibliography.bib network.pdf flow.pdf aceflow.pdf fig-network.tex fig-revproxy.tex fig-aceflow.tex
	pdflatex $<
	bibtex document
	pdflatex $<
	pdflatex $<

bibliography.d/auto/rfc%.bib:
	wget https://datatracker.ietf.org/doc/rfc$*/bibtex/ -O $@

bibliography.d/auto/draft-%.bib:
	wget https://datatracker.ietf.org/doc/draft-$(shell python3 -c 'print("$*"[::-1].replace("-", "/", 1)[::-1])')/bibtex -O- | sed '0,/a/ s/{/{draft-/' > $@

RFCS = $(shell grep -o rfc.... body.tex )
DRAFTS = $(shell grep -o 'draft-[a-z0-9-]\+' body.tex )

bibliography.bib: $(patsubst %,bibliography.d/auto/%.bib,$(RFCS)) $(patsubst %,bibliography.d/auto/%.bib,$(DRAFTS)) bibliography.d/auto/cost-of-oscore.bib $(wildcard bibliography.d/*.bib)
	cat $^ > $@

bibliography.d/auto/%.bib:
	wget ${URL} -O- | sed '0,/a/ s/{.*,/{$*,/' > $@

bibliography.d/auto/cost-of-oscore.bib: URL=https://dblp.uni-trier.de/rec/journals/corr/abs-2103-13832.bib?param=1

%.pdf: %.svg
	inkscape $< -o $@

